CHAMP: Characterizing Undesired App Behaviors from User Comments based on Market Policies

Millions of mobile apps have been available through various app markets. Although most app markets have enforced a number of automated or even manual mechanisms to vet each app before it is released to the market, thousands of low-quality apps still exist in different markets, some of which violate the explicitly specified market policies.In order to identify these violations accurately and timely, we resort to user comments, which can form an immediate feedback for app market maintainers, to identify undesired behaviors that violate market policies, including security-related user concerns. Specifically, we present the first large-scale study to detect and characterize the correlations between user comments and market policies. First, we propose CHAMP, an approach that adopts text mining and natural language processing (NLP) techniques to extract semantic rules through a semi-automated process, and classifies comments into 26 pre-defined types of undesired behaviors that violate market policies. Our evaluation on real-world user comments shows that it achieves both high precision and recall ($>0.9$) in classifying comments for undesired behaviors. Then, we curate a large-scale comment dataset (over 3 million user comments) from apps in Google Play and 8 popular alternative Android app markets, and apply CHAMP to understand the characteristics of undesired behavior comments in the wild. The results confirm our speculation that user comments can be used to pinpoint suspicious apps that violate policies declared by app markets. The study also reveals that policy violations are widespread in many app markets despite their extensive vetting efforts. CHAMP can be a \textit{whistle blower} that assigns policy-violation scores and identifies most informative comments for apps.

==> RQ4.tex <==

%%\iffalse
\vspace{-0.1in}
\subsection{RQ4: Market Reaction to Such Comments}

%%So far, the study results suggest the prevalence of undesired behavior comments, and pinpoint the difference across markets. 
We then seek to take a step further to understand how app markets react to such feedback for improving app regulations.
\eat{
To that end, we formulate three sub research questions here: \textbf{(RQ4.1) How quickly does each app market react to undesired behavior comments? }
As we have identified such comments from different markets, it is interesting to measure the response time for each of them and make a comparison.
\textbf{(RQ4.2) Are there any difference across the summarized behaviors?} As we have summarized five types of behaviors, we want to know the importance and severity of different types of behaviors from the view of app market maintainers. In common sense, the security behaviors would cause serious impacts and thus should be more concerned by app markets. We seek to verify this hypothesis.
\textbf{(RQ4.3) What are the general patterns of undesired behavior comments in the corresponding apps?} we want to know whether they were concurrently raised by app users, or they have intensive occurrence within a short period.
}
In particular, we measure the response time for each undesired behavior and make a comparison across all markets.
We also investigate the severity of different types of undesired behaviors from the view of app market maintainers, \ie how quickly an app is removed given the presence of a certain type of undesired behavior comments. 
%Intuitively, we expect the security-related behaviors would cause more impacts and thus should be more concerned by the app markets. We seek to verify this hypothesis.
%%Finally, we summarize the general patterns of undesired behavior comments in representative apps.

To perform these measurements, we need to get the comments posted during the \emph{whole life-cycle} for the studied apps. 
Thanks to Kuchuan, we can do that for the 8 Chinese app markets.
However, for Google Play, since we crawled the comments by ourselves, we were unable to collect the comments for the apps' whole life-cycle.
Therefore, in this measurement, we study only the Chinese markets.


% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.3\textwidth]{figure/malwarereactiontime1.pdf}
% % \vspace{-0.1in}
% \caption{Distribution of reaction time across markets.}
% % \vspace{-0.2in}
% \label{fig:reaction-time}  
% \end{figure}

\begin{figure}[t]
	\centering
	\subfigure[Distribution of reaction time across markets.]{
		\label{fig:reaction-time}
		\includegraphics[width=0.22\textwidth]{figure/malwarereactiontime1.pdf}}
%  	\hspace{0.2ex}
	\subfigure[Reaction time across different undesired behaviors]{
		\label{fig:allMarketsPercentage}
		\includegraphics[width=0.22\textwidth]{figure/allmarkets1.pdf}}
\vspace{-0.15in}
	\caption{Comparing the reaction time from (a) app markets (b) behavior types}
\end{figure}

\textbf{RQ4.1: Market Reaction Time.} 
%%For a given app $APP_{i}$ and the hosting market $Market_{n}$, 
We calculate the reaction time of $Market_{n}$ to app $APP_{i}$ as the period between \emph{the first identified undesired behavior comment} and \emph{the app removal in the market}, as shown in Figure~\ref{fig:reaction-time}.
%, We obtain several observations. 
First, in general, all the studied markets take an unexpected long time to remove policy-violation apps, \eg the average time is 761 days. 
Second, the reaction time varies across markets. 
For example, Huawei has the shortest reaction time on average (362 days), while 360 Market has the longest reaction time on average (1393 days). 
%%Nevertheless, all the studied markets take unexpected long time to remove the policy-violation apps. 
Third, the variance of reaction time for apps in a single market is very large. 
For example, the reaction time for apps in Tencent varies from 0 days to 2324 days. 
\textbf{This suggests that app markets have not taken advantage of user comments to facilitate the app maintenance process, while \tool could positively provide insights for the app market maintainers and help them identify potential undesired behaviors and malicious apps accurately and timely}.
%%\textbf{\emph{although there exists subtle difference across markets, app markets seem not to take explicit actions to respond to the undesired behaviors proactively.}} The major reason might be that, 


\textbf{Market Reaction Time Across Different Behaviors.} 
% Towards verifying the hypothesis that app markets would react to various types of undesired behaviors differently, we further analyze the reaction time from the view of behaviors. 
As we have categorized the undesired behaviors into five categories (cf. Section~\ref{sec:background}), we measure the percentage of the removed apps for a given behavior category across time, shown in Figure~\ref{fig:allMarketsPercentage}.
% As shown in Figure~\ref{fig:allMarketsPercentage}, it is obvious that different behaviors diverse greatly. 
In general, the apps with security-related behaviors were removed a little quicker than other apps. 
Over 87\% of them were removed in 1230 days. 
As a comparison, the percentage for illegitimate behavior category is 73\%.
\textbf{This suggests that there is no strong correlation between the undesired behavior types and the current reaction time for app markets. With the help of \tool, it will be possible to pinpoint more urgent violations accurately, such as security-related ones, so that the markets could choose their reaction accordingly.}
%%\textbf{Although with no strong correlation (as the reaction time is long in general), we believe that the undesired behaviors would impact the reaction time to some extent. }

\iffalse
\textbf{RQ4.2: General Patterns.} 
To study the general patterns of apps with undesired behavior comments, we randomly select 100 apps (20 apps for each behavior, with no overlap), and then plot the trend of undesired behavior comments for each of them. 
Taking efforts to manually examine all of them, we  summarized two general patterns, as shown in Figure~\ref{fig:casestudy}. 

For apps in the first trend (cf. Fig.~\ref{fig:casestudy}(1)), in their initial stage, only a few users download them and both the comments and undesired behavior comments are not many. 
However, in their later stage, with the growth of the users or with the upgrades of apps, a large number of user comments were posted, and the undesired behavior comments increase as well.
For example, for the app ``com.dalongtech.cloud'', over 750 undesired behavior comments were found in 2018, and then the app was removed from the markets. 
This suggests that the app developers fail to address the increasing complaints from the users and the app was removed. 
The other pattern has an opposite trend (cf. Fig.~\ref{fig:casestudy}(2)). 
The number of undesired behavior comments reaches a peak at an intermediate stage, and then drops quickly. 
In the end, there were almost no comments.
In this case, the possible reason is that, after too many people complained about the app, few new users downloaded and commented the app, and then it was removed due to inactivity.
\fi


   

%%In this section, the removed duration of apps is calculated according to the behaviors of each app. For example, for each app, the latest time data demonstrates the date when the app is removed. Similarly, the most early date of each behavior of this app can be also found in database system. After that, the time difference between the two date shows how long time the behavior is reported in comments at the beginning until the app is removed. Hence, each behavior duration of an app can be seen clearly which means the behavior with the shortest duration demonstrates that the behavior is cared much more than other behavior in this app store. For instance, if in 360 store, the 'fail to install' behavior has the shortest duration, it says that the 'fail to install' behavior is cared most for store 360. Furthermore, the time data can help to see which app store reacts faster and which behaviors are cared much in every store.

%%\subsubsection{Response time in each app market statistic }

%%To see which market has the most fast response time towards the users negative feedback, the boxplot figure can show the comparison more clearer than other techniques. The figure~\ref{fig:markets} shows the average app removing time in each app market. The figure is generated by boxplot. For each app market, the durations from the first comment of each malicious behavior to the last comment of this app are as the input data for the boxplot so this figure can demonstrate the average response time for every malicious behavior in each market. In this figure, the x-axis is the app markets while the y-axis shows the removing time which the unit is days. As we can see in the figure, market oppo has the most fast response time and duration. For oppo, the average reaction time is less than 300 days and the duration is about 400 days, which is the least among all markets. The next two markets who response faster than others are meizu and huawei. The app market 360 owns the most slowest reaction time towards users negative feedback.The reaction time is around 1250 days. But the market yingyongbao has the most long duration. The duration is about 1000 days. The figure~/ref{fig:allMarketsPercentage}shows the numbers of removed app with each malicious behaviors that occupied how much percent in the whole apps matched negative behaviors during 30 to 1830 days. Each line shows a kind of behavior. It can be divided into 3 groups. The first group is the behavior which is cared mostly by markets. They are ads, fail to start and vulgar. They are over 40 percents occupied in the whole apps which is higher than other behaviors. For ads behavior, it reaches to 60 percents almost. The markets take faster response time to the three behaviors. The markets take middle speed to the second group behaviors. For the figure, they are virus, direct to other websites, fail to log in and fail to uninstall. They occupied from 10 percent to 30 percent among the whole app numbers. The markets do response for them, but not as fast as the behaviors in first group. For the third groups, the markets take very slow response time for them. They only occupied less than 10 percent among the apps. They are illegal authorization, fail to retrieve content and malicious hidden. The markets response slowly to them, it might also be that the users cannot realize the behaviors easier than the behaviors in the former two groups. From this figure, it can tell us that which kinds of behaviors make more sense for users and markets.
%%\subsubsection{Case study: relationship between time, behaviors and percentage}
%%To understand if the markets indeed have done some actions to improve the app quality or pay enough attention on users negative feedback, some case studies are done to show the relationship between removing time, comments numbers or removing app numbers. As we can see from the figure~\ref{fig:casestudy}, the figure (a) and (b) shows two apps comments number decreasing and increasing trend through years from when the app comes out to the app has been removed. For the figure (a), the every year all comments and negative comments of app 'com.dalongtech.cloud' shows an increasing trend. It might be like that through the days more and more users would write comments to report the negative sides of the app. Because the app does contain positive functions, people still use it but write the comments below. That is why the comments and negative comments number shows an increasing trend. On the contrast, for the figure (b), it shows a decreasing trend. Especially in 2017 and 2018, it drops sharply. It might because the app shows many negative actions which is more than the positive functions so that users decided to leave this app. That is why both the numbers of the all comments and negative comments drop sharply. 
%\subsubsection{Removing time of each behaviors statistic }
%Moreover, the box plot tool can show the removing time of each behaviors among all app markets clearly to demonstrate which kinds of behaviors are cared much more than other behaviors and which types of behaviors are less focused by markets. The figure~\ref{fig:behaviors} shows the average removing time of each malicious behaviors. For each box, the input data is that each average removing time of each behavior at each app market. From this figure, the first 6 malicious behaviors from fail to install to fail to login have close average removing time which is around 850 days. But it is obvious to see that the virus behavior has the most short removing duration and time in all app markets. It only takes about average 500 days to remove an app has comments about virus and the removing time duration is less than 100 days.  The next two behaviors has the least removing time is force to download other apps and illegal operation on background, the average removing time is about 600 days, while the behavior force to download other apps has less duration. The behavior too many ads has the longest removing time and the behavior fail to start has the longest duration which is 1150 days and 1400 days respectively. The apps who do match any malicious behaviors are counted. The removing time of those apps are as the input data. It can be seen that the apps who do not match behaviors has the removing time which is about 700 days, which is less than half of the app behaviors. But it has the 1000 days removing duration which is longer than half of the behaviors.
% \subsubsection{Case study: relationship between time, behaviors and percentage}
% To understand if the markets indeed have done some actions to improve the app quality or pay enough attention on users negative feedback, some case studies are done to show the relationship between removing time, comments numbers or removing app numbers. 
% \item \emph{\textbf{Case study No.1: the removing app percentage and removing time}} In this study, the relationship between removing time and removing app numbers among all apps in each specific behaviors at all market. As can be seen in figure~\ref{fig:allMarketsPercentag}, the x-axis is the removing days and the y-axis means that how many percentage  the removed app numbers occupied in the all app numbers of each behaviors. For example, as can be seen, at 30 days, about 38 percents apps which has direct to other websites are removed. This figure shows that at 1830 days, most types of behaviors which the apps have been dealt and  removed from the market while the behaviors ads and inconsistency are not. Only 82 percents apps are removed in  1830 days for this two behaviors. It is obvious to see that the behaviors direct to other websites, fail to start and force to download has a sharper increasing than other curves. They reach to 100 percents faster than other behaviors. Hence the three behaviors are cared more than other behaviors. Seems the behaviors steal privacy, fail to exit, and vulgar are less cared by the markets. All of them do not have a high percentage at the first 630-930 days, while other behaviors own the reaction time at the first 630 days.
% \item \emph{\textbf{Case study No.2: some specific apps}} In this section, some apps which have most numbers of negative comments or most numbers of negative behaviors labels are picked to be studied. For those figures, all of them have x-axis is the year while the y-axis is the numbers of comments. The figure~\ref{fig:maxNegativeComments}
% shows two apps which have the most numbers of negative comments. As can be seen, the two apps show a decreasing trend of the negative comments numbers. The first app reaches a peak at 2014 and decreased to about 1 at 2016 year. The second app shows a decreasing trend as well but it fluctuates. It reaches the peak at 2016 around 36 and drops to 1 at 2018. Similarly, the next two apps in figure~\ref{fig:maxTypeOfNegativeComments} shows the decreasing trend too. The two apps match the most type numbers of malicious behaviors. But the first app reaches the peak at 25 negative comments numbers and finally drop to about 2 at 2015. The second app only exist at 2015 with 31 negative comments and then be removed from the market. As a conclusion, the app markets do have done reaction towards the apps contains negative comments which contains malicious behaviors.
% \item \emph{\textbf{Case study No.3: time and numbers of grey behaviors and malicious behaviors}}In this section, a case study about the relationship between the timeline and numbers of grey behaviors and malicious behaviors has been done to research the app markets response ability. The grey behaviors means the behaviors are not malicious but it also violates the market policies, like too many ads. For the first figure~\ref{fig:com.dalongtech.cloud}, obviously both the grey and malicious behaviors have the increasing trend along the years. At Oct-2018, the grey behaviors reach the peak at 180 numbers. For the malicious behavior, at about June-18, it reaches the peak around 120 numbers. Both of them reach the peak at 2018.
% For the second figure~\ref{fig:com.ezjoy.feelingtouch.zombiediary2China}, we can see that the malicious behavior shows a decreasing tendency. It drops from 20 and then reach to 32 around 10/2014, then continues to drop to 3 at around 11/2018. For the grey behaviors, it fluctuates and then back to the begining. It starts from 20 at 6/2014 and reach to the peak at 45 at around 10/2014, after that it drops to 5 at 8/2015 then go back to 12 at around 11/2018 while before that it jumps to 40.
% For the second figure~\ref{fig:com.QQ.angel.webApp},the grey behaviors shows an increasing trend. It fluctuates at the beginning, then jumps to 300 at 9/2017 after that it reaches the peak at 450 at July-2018 and then decreased to 70 at Oct-18. But this app does not have much malicious behaviors, it almost stay around 1 or 2 all the time.




% \label{sec:methodlogy}
% \begin{figure*}
% \centering
%   \includegraphics[width=1.1\textwidth]{figure/bandn.jpg}
% \vspace{-0.1in}
% \caption{The average removing time of each behaviors.}
% \vspace{-0.2in}
% \label{fig:behaviors}       % Give a unique label
% \end{figure*}

% \begin{figure}
% \centering
%   \includegraphics[width=0.32\textwidth]{figure/allmarkets.pdf}
% % \vspace{-0.1in}
% \caption{Reaction time across different undesired behaviors.}
% % \vspace{-0.2in}
% \label{fig:allMarketsPercentage}       % Give a unique label
% \end{figure}


\iffalse
\begin{figure}
\centering
  \includegraphics[width=0.49\textwidth]{figure/casestudy.pdf}
 \vspace{-0.2in}
\caption{Two general patterns of undesired comments.}
% \vspace{-0.2in}
\label{fig:casestudy}       % Give a unique label
\end{figure}
\fi
%%\fi

